Oriented Matroids and Combinatorial Neural Codes

A combinatorial neural code $\mathscr C\subseteq 2^{[n]}$ is convex if it arises as the intersection pattern of convex open subsets of $\mathbb R^d$. We relate the emerging theory of convex neural codes to the established theory of oriented matroids, both categorically and with respect to geometry and computational complexity. On the categorical side, we show that the map taking an acyclic oriented matroid to the code of positive parts of its topes is a faithful functor. We adapt the oriented matroid ideal introduced by Novik, Postnikov, and Sturmfels into a functor from the category of oriented matroids to the category of rings; then, we show that the resulting ring maps naturally to the neural ring of the matroid's neural code. For geometry and computational complexity, we show that a code has a realization with convex polytopes if and only if it lies below the code of a representable oriented matroid in the partial order of codes introduced by Jeffs. We show that previously published examples of non-convex codes do not lie below any oriented matroids, and we construct examples of non-convex codes lying below non-representable oriented matroids. By way of this construction, we can apply Mn\"{e}v-Sturmfels universality to show that deciding whether a combinatorial code is convex is NP-hard.

==> section-5.tex <==


\section{Non-convex codes} %Codes -> codes per Y 10
\label{sec:non_convex}

Though it is unknown whether every convex code has a realization with convex polytopes, the contrapositive to Theorem~\ref{thm:polytope_matroid} helps us characterize non-convex codes. 
If $\scC$ is not convex, one of two possibilities hold: either $\scC$ does not lie below any oriented matroid,
or $\scC$ lies below only non-representable oriented matroids in $\pcode$.
In this section, we prove that codes with local obstructions as well as
``sunflower codes''
do not lie below {\em any} oriented matroids. We also construct a new class of
non-convex codes which lie below non-representable oriented matroids.


%The contrapositive of Proposition \ref{prop:no_local} implies the following result:
%
%\begin{prop}
%  If $\scC$ is a code with a local obstruction, then $\scC$ does not lie
%  below any oriented matroid code.
%\end{prop}

\subsection{Sunflower codes do not lie below oriented matroids}

The first example of a non-convex code with no local obstructions,
	\[ \scC = \{2345, 123, 134, 145, 13, 14, 23, 34, 45, 3, 4, \emptyset\}, \]
appeared in \cite{lienkaemper2017obstructions}. In \cite{jeffs2019morphisms}, Jeffs uses this code to construct a smaller non-convex code $\scC_2 \leq \scC$ with no local obstructions,
	\[ \scC_2 = \{1236,   234, 135, 456, 23, 13,4, 5, 6, \emptyset  \}. \]
This code  is minimally non-convex, in the sense that any code $\scC' \leq \scC_2$ in $\pcode$ is convex. The proofs that $\scC$ and $\scC_2$ are not convex depend on
% the following lemma: 
the $n=3$ case of the following theorem:

%\begin{lem}[\cite{lienkaemper2017obstructions}, Lemma 3.2] Let $U_1, U_2, U_3$ be convex open sets in $\R^2$ such that for $U_1\cap U_2 = U_2\cap U_3 = U_1\cap U_3 = U_1\cap U_2 \cap U_3$. Then any line which passes through $U_1, U_2$, and $U_3$ passes through $U_1\cap U_2 \cap U_3$. 
%\end{lem}
%
%
%
%
%In \cite{jeffs2019sunflowers}, this result is generalized to the following theorem:

\begin{thm}[\cite{jeffs2019sunflowers}, Theorem 1.1] \label{thm:sunflower} Let $U_1, \ldots, U_n$ be convex open sets in $\R^{n-1}$ such that for all $i, j\in [n]$, $U_i \cap U_j = \bigcap_{k\in [n]} U_k$. Then any hyperplane which passes through $U_1, \ldots, U_n$  passes through $\bigcap_{k\in [n]} U_k$. 
\end{thm}

Jeffs uses this theorem to construct an infinite family $\{\scC_n\}_{n\geq 2}$ of minimally non-convex codes with no local obstructions generalizing $\scC_2$; we refer to these as ``sunflower codes.'' In the rest of this subsection, we define the code $\scC_n$ for $n\geq 2$ and give a proof that for all $n\geq 2$, the code $\scC_n$ does not lie below any oriented matroid, representable or otherwise. 

\begin{defn}[\cite{jeffs2019sunflowers}, Definition 4.1]
  Let $n \geq 2$, $P = \{p_1,\ldots,p_{n+1}\}$ and $S = \{s_1,\ldots,s_{n+1}\}$ be sets of size $n+1$.
Denote by $\scC_n \subseteq 2^{P\cup S}$ the code that consists of the following codewords: 
\begin{itemize}
	\item $\varnothing$; 
	\item $S \cup \{p_{n+1}\}$; 
	\item $P$;
	\item the codeword $X \cup \{s_{n+1}\}$  for each $\varnothing \subsetneq X \subsetneq \{s_1,\dots,s_n\}$;
	\item the codewords $\{p_i\}$ for each $1 \leq i \leq n+1$;
	\item and $(S \setminus \{s_i\}) \cup \{p_i\}$ for each $1 \leq i \leq n$. 
  \end{itemize}
\end{defn}

We will refer to the regions indexed by $P$ as {\em petals},
and the regions indexed by $S$ as {\em simplices}.
\begin{figure} [ht!]
	\includegraphics[width = 4 in]{C2GoodCover.pdf}
	\caption{A good cover realization of $\scC_2~=~\{\emptyset, 23, 13, 4, 5, 6, 234, 135,  1236, 456\}.$ Here $P = \{1,2,3\}$ and $S = \{4,5,6\}$.} 
\end{figure}

The proof of  \cref{thm:bad_sunflower} depends on some basic facts about tope graphs of oriented matroids. The \emph{tope graph} $\cT$ of an oriented matroid $\cM$ is a graph whose vertices are the topes of $\cM$, and whose edges connect pairs of topes which differ by one sign. A subgraph $\mathcal Q \subseteq \cT$ is called $T$-convex if it contains the shortest path between any two of its members. Any $e\in E$ divides the tope graph into two \emph{half-spaces} $\cT_e^+ = \{W\in \cW \mid  e\in W^+\}$ and $\cT_e^- = \{W\in \cW \mid  e\in W^-\}$.
A subgraph $\cQ \subseteq \cT$ is $T$-convex if and only if it is an intersection of half-spaces \cite[Proposition 4.2.6]{bjorner1999oriented}.
%Our proof uses Proposition 4.2.6 of \cite{bjorner1999oriented}: a subgraph $\mathcal Q \subseteq \cT$ is $T$-convex if and only if it is the intersection of half-spaces. 

\begin{introtheorem}
	For each $n \geq 2$, the code $\scC_n \not \leq \sfL^+\cM$ for any oriented matroid $\cM$.
\end{introtheorem}

\begin{proof}
Fix $n \geq 2$.
Suppose to the contrary that there is an oriented matroid $\cM$ such that $\scC_n \leq \sfL^+\cM$.
For ease of notation, let $\scM$ denote the code $\sfL^+\cM$.
Since $\emptyset \in \scC_n$, we can assume without loss of generality that  $\scC_n = f(\scM)$  for some code morphism $f$.


Denote the ground set of $\cM$ by $E$. The map $f$ must be defined by
trunks
	 \[\tk_{\scM}(\pi_1), \dots, \tk_{\scM}(\pi_{n+1}), \tk_{\scM}(\sigma_{1}), \ldots,\tk_{\scM}(\sigma_{n+1}),\]
with $\pi_i,\sigma_i \subseteq E$ corresponding to $p_i$ and $s_i$ respectively. 

\vspace{3mm}
\noindent  {\bf Claim 1:} There is a tope $T$ of $\cM$ such that
    $\left(\bigcup_{i=1}^{n+1} \s_i\right)\cup \left(\bigcap_{j=1}^{n} \pi_j\right)\cup \pi_{n+1} \subseteq T^+$.\\
  Roughly speaking, we are producing a codeword in the intersection of the
  last petal and all simplices, which also lies in the convex hull of the other petals.
  
Define a morphism $g:\scM \to 2^{[n+1]}$ by the trunks $T_i = \tk_{\scM}(\tau_i)$, with 
$\tau_i = \sigma_i \cup \left(\,\,\bigcap_{j = 1}^{n}{ \pi_j}\,\right)$ for $i = 1, \ldots, n+1$.
Let $\scD = g(\scM)$.


Since $(S \setminus \{s_i\} )\cup \{p_i\} \in \scC_n$ for each $i \in [n]$, we deduce that $[n+1]\setminus i$ is a codeword of $\scD$ for each $i\in [n]$. Thus, $\link_{\{n+1\}}(\Delta(\scD))$ is either a hollow $(n-1)$-simplex or a solid $(n-1)$- simplex. Since we have defined $\scD$ as the image of an oriented matroid code, it cannot have local obstructions.
The codeword $\{n+1\}$ is not in $\scD$; if it were, then $f(g^{-1}(\{n+1\}))$
would be a codeword of $\scC$ including $s_{n+1}$ without any other $s_i$. No such codeword
exists in $\scC$.
Thus $\link_{\{n+1\}}(\Delta(\scD))$ must be contractible. Because $\{n+1\}$ is not a codeword of $\scD$,  the $\link_{\{n+1\}}(\Delta(\scD))$ must be a solid $(n-1)$-simplex; therefore, $[n+1]$ is a codeword of $\scD$. 

Based on the trunks defining $g$, we know that
$\left(\bigcup_{i =1}^{n+1}\sigma_i\right) \cup \left( \bigcap_{j = 1}^{n} \pi_j \right)\subseteq g^{-1}([n+1])$.
By definition of $f$, we must also have $S \subseteq f(g^{-1}([n+1]))$; however, the only codeword of $\scC_n$ which contains $S$ is $S \cup \{p_{n+1}\} $.
Thus, there is a codeword of $\scM$ containing $\left(\bigcup_{i =1}^{n+1}\sigma_i\right)
\cup \left(\bigcap_{j = 1}^{n} \pi_j \right)\cup \pi_{n+1}$. This implies that
$\cM$ has a covector $X$ such that 
 $\left(\bigcup_{i =1}^{n+1}\sigma_i\right)
\cup \left(\bigcap_{j = 1}^{n} \pi_j \right) \cup \pi_{n+1} \subseteq X^+$. To produce a tope satisfying the condition, take $T = X\circ W$ for any tope $W$ of $\cM$. 


\vspace{3mm}
  
\noindent  {\bf Claim 2:}
$ \pi_{n+1} \cup \left( \,\,\bigcap_{ j=1}^{n}\,\pi_j\right) \subseteq T^+ $   implies $\,\,\bigcup_{ j=1}^{n+1}\,\pi_j \subseteq T^+ $ for any tope $T$ of $\cM$.\\
The intuition here is that the last petal must intersect the convex
hull of the other petals {\em only} in the common intersection of all petals.

\begin{figure}
\includegraphics[width = 2.5 in]{non_mat_proof_fig.pdf}
\caption{Any path from a tope $U$ with $\left(\bigcup_{ j=1}^{n+1}\,\pi_j\right) \subseteq U^+$ to a tope $V$ with $\left(\bigcup_{ j=1}^{n+1}\,\pi_j\right) \not\subseteq V^+$ must cross an edge in  $\left(\bigcap_{ j=1}^{n+1}\,\pi_j\right)$. Analogously, a path from a point in the atom $P = \{p_1, p_2, \ldots, p_n\}$ to the atom $\{p_{n+1}\}$ must cross the boundaries of $p_1, p_2, \ldots, p_{n}$ all at one time. }
\end{figure}

Let $U$ be a tope with $\left(\bigcup_{ j=1}^{n+1}\,\pi_j\right) \subseteq U^+$. Such a tope must exist, since $P \in \scC_n$.   Suppose for the sake of contradiction that there exists a tope $V$ such that 
\[
\pi_{n+1} \cup \left( \,\,\bigcap_{ j=1}^{n+1}\,\pi_j\right) \subseteq V^+, \text{   but   }\bigcup_{ j=1}^{n+1}\,\pi_j \not \subseteq  V^+.
\]
Consider a shortest path from $U$ to $V$ in the tope graph of $\cM$.  Each edge of the tope graph is naturally labeled by the ground set element $e$ by which the two incident topes differ.  By the $T$-convexity of intersections of half-spaces in the tope graph, each tope along this path has
$\pi_{n+1} \cup \left( \,\bigcap_{ j= 1}^{n}\,\pi_j\right) $ in its positive part, so no edge is labeled with an element of $\bigcap_{ j=1}^{n}\,\pi_j$. 

Thus at some point along the path from $U$ to $V$, we must cross an edge $(T, W)$ labeled by a ground set element 
$e \in
\left(\,\,\bigcup_{ j=1}^{n+1}\,\pi_j \right) \setminus
\left(\,\,\bigcap_{ j=1}^{n+1}\,\pi_j \right)$.
Choose the first such edge  $(T, W)$ labeled with ground set element $e$. By our choice of $e$, there exist
$k, \ell \in [n]$ such that $e\in \pi_k$, and $e\notin \pi_\ell$.
This means $\pi_k \not\subseteq W^+$, whereas $\pi_\ell \subseteq W^+$. Then
$\{p_\ell, p_{n+1}\} \subseteq f(W^+)$, but $f(W^+) \neq P$. However, the only codeword of $\scC_n$ containing $\{p_\ell, p_{n+1}\}$ is $P$, so we have reached a contradiction.
Therefore, no such tope $V$ may exist.

\vspace{6mm}
 

\noindent By Claim 1, $\cM$ must have a tope $T$ which has
$\left(\bigcup_{i=1}^{n+1} \s_i\right)\cup \left(\bigcup_{j=1}^{n} \pi_1\right)  \cup \pi_{n+1} \subseteq T^+$.
Because $T$ satisfies
$\left(\bigcap_{i=1}^{n+1} \pi_i\right) \cup \pi_{n+1} \subseteq T^+$, Claim 2 implies
that $\bigcup_{i=1}^{n+1} \pi_i \subseteq T^+$.
Therefore,
$\left(\bigcup_{i=1}^{n+1} \pi_i\right) \cup \left(\bigcup_{i=1}^{n+1} \s_i\right) \subseteq T^+$,
but this implies $f(T) = P\cup S \in \scC_n$, a contradiction. 
\end{proof}

By showing that the family of codes $\{\scC_n\}_{n\geq 2}$ do not lie below oriented matroids, we have given an alternate proof that these codes do not have realizations with interiors of convex polytopes.
 This proof is significantly different in structure than the original proof that these codes are not convex using \cref{thm:sunflower}, which is in turn proved by induction on dimension. 
 In contrast, our proof makes no reference to rank or dimension, and does not use induction. 
 While the codes $\{\scC_n\}_n$ are not open convex, they do have realizations with \emph{closed} convex sets, which can even be chosen to be (non-full dimensional) closed convex polytopes. 
 Notice that  \cref{thm:polytope_matroid}  establishes that if $\scC$ has a  realization with \emph{interiors} of convex polytopes, then  $\scC \leq \sfL^+\cM$. 
 However, the fact that a code has a realization with closed convex polytopes does not guarantee this. 
 Further, in showing that these codes do not lie below any oriented matroids at all, we have established that, even while these codes are good cover codes, their obstructions to convexity are somehow still topological in nature. 

\subsection{Representability and convexity}
Having exhibited that many well known non-convex codes do not lie below any oriented matroids at all, we now exhibit a family of non-convex codes which lie below non-representable matroids.
  For the remainder of this section, we consider $\sfL^{\pm}(\cM)$, the code on $2n$ neurons
  with a codeword $X^+ \sqcup X^-$ for each covector $X$. (Notice that this is really just the set $\cL(\cM)$, viewed as a code on $\pm E$.) We will prove that a uniform
  oriented matroid $\cM$ is representable if and only if
  $\sfL^{\pm}(\cM)$ is a convex neural code. 
This theorem helps describe a new infinite family of non-convex codes with no local obstructions. 

This result also shows that the decision problem of determining whether an oriented matroid is representable is a special case of the decision problem of determining whether a code is convex. This proves that the computational complexity of checking matroid representability provides a lower bound to the complexity of determining whether a code is convex.
First we prove the following necessary lemma:

\begin{lem} \label{lem:tope_lemma} If $X = X^+ \cup X^-$ is a covector of a uniform affine oriented matroid $\cA$ on $[n]$, and $U\in \{+, -\}^n$, then $X\circ U$ is a tope of $\cA$.  
\end{lem}

\begin{proof}
Let $(\cM, g)$ be an oriented matroid such that $\cA = \cM_g$. Since $X$ is a covector of $\cM$, it is a restriction of a tope of $\cM$. By \cite{lawrence1983lopsided} (in the notation of Exercise 3.28 of \cite{bjorner1999oriented}), either there is a tope $T$ such that $X\circ T\in \cW$ but $X\circ -T \notin \cW$, or  $X\circ U$ is a tope of $\cM$ for all $U\in \{+, -\}^n$. Since $X$ is a covector,  $X\circ T\in \cW$ and $X\circ -T \in  \cW$ for all topes $T$. Thus we must instead have that $X\circ U$ is a tope of $\cM$ for all $U\in \{+, -\}^n$. Since $X_g = +$, $(X\circ U)_g = +$, so $X\circ U$ is a tope of $\cA$. \end{proof} 



\begin{introtheorem}
	Let $\cM = (E, \cL)$ be a uniform oriented matroid. Then $\cM$ is representable if and only if the code $\sfL^\pm(\cM) \subseteq 2^{\pm E}$ is convex.  
\end{introtheorem}

\begin{figure}
	\includegraphics[width = 4 in]{witness3.pdf}
	\caption{Hyperplane realization constructed from convex code realization
	  as in the proof of Theorem \ref{thm:witness}.   }
\end{figure}




\begin{proof}
First, suppose $\cM = (E, \cL)$ is representable. Let $\{H_e\}_{e\in E}$ be a hyperplane arrangement representing $\cM$. For each $e\in E$, let $U_e = H_e^+$ and $U_{\bar e} = H_e^-$. Then by the definition of the oriented matroid of a hyperplane arrangement, $\code(\{U_e\}_{e\in E} \cup \{ U_{\bar e}\}_{e\in E} ) = \sfL^{\pm}(\cM)\subseteq 2^{\pm E}$. Thus $\sfL^{\pm}(\cM)$ is a convex code.  

\vspace{3mm}

Conversely, suppose $\sfL^{\pm}(\cM)$ is a convex code.
Note that it is sufficient to prove that, for any $g\in E$, the affine oriented matroid $\cM_g$
is representable: taking the cone over the realization of $\cM_g$ by the origin
yields a realization of $\cM$.
Let $g\in E$, and let $\cA = \cM_g$ be the affine oriented matroid with
$\sfL^{\pm}(\cM_g) = \{X\in \sfL^{\pm}(\cM) \mid X_g = +\}$.
Because trunks of convex codes are convex, $\sfL^{\pm}(\cM_g^+) \cong  \tk_{\sfL^{\pm}(\cM)}(g) $ is convex.

Let $\{U_e\}_{e\in E\setminus g} \cup \{U_{\bar e}\}_{e\in E\setminus g}$
be a convex realization of $\sfL^{\pm}(\cM_g^+)$. %in an ambient space $\R^k$.
For each $e$, the sets $U_{e}$ and
$U_{\bar e}$ are disjoint convex open sets. Thus, by the hyperplane separation theorem,
for each $e$, there is a hyperplane $H_e$ separating $U_{e}$ and $U_{\bar e}$.
Let $\cA_H$ be the affine oriented matroid of the hyperplane arrangement
$\{H_e\}_{e\in E\setminus g}$. By construction, $\cA_H$ is representable.
We claim that $\cA_H = \cA$. To show this, it is sufficient to check that
$\cA$ and $\cA_H$ have the same cocircuits.


Let $X = (X^+, X^-)$ be a cocircuit of $\cA$ and $\sigma = E\setminus \underline{X}$.
By Lemma \ref{lem:tope_lemma}, $X\circ U$ is a tope of $\cA$ for each $U\in \{+, -\}^E$.
Thus, for each of the $2^{|\sigma|}$ subsets $\tau \subseteq \sigma$,
there is a codeword $c$ of $\sfL^{\pm}(\cM_g)$  with $e \in c$ for all $e\in \tau$, $\bar f\in c$ for all $f\in \sigma \setminus \tau$. Thus for all $\tau \subseteq \sigma$, 
\[\left(\bigcap_{e\in \tau} U_e \right) \cap \left(\bigcap_{f\in \sigma \setminus \tau} U_{\bar f}\right)\neq\emptyset; \text{   consequently,   } \left(\bigcap_{e\in \tau} H_e^+ \right) \cap \left(\bigcap_{f\in \sigma \setminus \tau} H_f^-\right)\neq \emptyset .\]
The $|\sigma|$ hyperplanes $\{H_e\}_{e\in \sigma}$ divide space into $2^{|\sigma|}$ regions,
which implies that they must all intersect. Therefore, $\bigcap_{e\in \sigma} H_e \neq \varnothing$.


For all points $p \in \bigcap_{e\in \sigma} H_e $, the associated codeword in $\sfL^{\pm}(\cM_g)$ includes
neither $i$ nor $\bar{i}$ for any $i \in \sigma$
since $U_i \cup U_{\bar{i}}  \subseteq H_i^+ \cup H_i^-$.
The only codeword of $\sfL^{\pm}(\cM_g)$ with this property is $\sfL^{\pm}(X)$, since $X$
is a cocircuit. We infer that
\[\bigcap_{e\in \sigma} H_e \subseteq \left[ \bigcap_{i \in X^+} H_i^+ \cap \bigcap_{j \in X^-} H_j^-\right].\]
Because this region is nonempty, $X$ is a covector of $\cA_H$. Furthermore,
because no $H_i$ for $i \notin \sigma$ intersects this region, $X$ is a minimal covector and therefore a cocircuit.


Thus, all cocircuits of $\cA$ are cocircuits of $\cA_H$.
Finally, since $\cA$ is uniform, each unsigned set
of size $n - r(\cA)+1$ is the support of a cocircuit of $\cA_H$. Therefore, by circuit axiom (C3),
$\cA_H$ can have no other cocircuits, meaning that $\cA = \cA_H$ as required.
\end{proof}

Theorem \ref{thm:witness} demonstrates that matroid representability and
convex code realizability are intertwined. One consequence is that
non-representable oriented matroids are a new source
for constructing non-realizable codes:

\begin{cor}
  There is an infinite family of non-convex codes which lie below
  oriented matroids in $\pcode$.
 \end{cor}

\begin{proof}
  There are infinitely many non-representable uniform oriented matroids $\cM$ \cite[Proposition 8.3.1]{bjorner1999oriented}. 
  By Theorem~\ref{thm:witness}, $\sfL^{\pm}(\cM)$ is non-convex for each of these.
  This code can also be obtained as $\sfL^+(\cM')$ where $\cM'$ is defined by doubled ground set
  $E \sqcup E'$ with corresponding elements anti-parallel.
\end{proof}

\begin{ex} Let $\cA = (\{1, \ldots, 9\}, \cL)$ be the uniform non-Pappus matroid from \cite{shor1991stretchability}. This matroid is non-representable, since a realization of it would violate Pappus's hexagon thoerem. Then $\cL$ is a non-convex code with no local obstructions. The code $\cL$ is the code of the cover $U_1, U_{\bar 1}, \ldots, U_9 , U_{\bar 9}$ depicted in Figure \ref{fig:non-papp}.

\begin{figure}[ht!]\label{fig:non-papp}
\includegraphics[width = 3.5 in]{non-papp.pdf}
\caption{This uniform non-Pappus arrangement defines a non-convex code $\cL \subset 2^{\pm [9]}$. This is the code
	\[ \cL = \code(\{U_1, U_{\bar 1}, \ldots, U_9 , U_{\bar 9}\}), \]
where $U_1, \ldots, U_6$ are the sets of points to the right of the lines labeled 1 through 6, $U_{\bar1}, \ldots, U_{\bar 6}$ are the sets of points to the left of the lines labeled 1 through 6,  $U_7, U_8,$ and $U_9$ are the sets of points below the pseudolines labeled 7, 8, and 9, and $U_{\bar 7}, U_{\bar 8},$ and $U_{\bar9}$ are the sets of points above the pseudolines labeled 7, 8, and 9.  }
\end{figure}

\end{ex}

\subsection{The convex code decision problem is NP-hard}

	We now turn to the computational aspects of convex codes.
	Using the relationship between convex codes and representable oriented matroids (Theorem~\ref{thm:witness}), we demonstrate the convex code decision problem is NP-hard and $\exists\R$-hard, though it remains open whether the convex code decision problem lies in either of these classes, or is even decidable.
	The complexity class $\exists \R$, read as \emph{the existential theory of the reals}, is the class of decision problems 
%	which ask if a sentence 
	of the form 
		\[ \exists (x_1\in \R) \ldots \exists(x_n\in \R) P(x_1, \ldots, x_n), \]
%	is true of false. In this definition, $P$ is a quantifier free formula whose 
	where $P$ is a quantifier-free formula whose atomic formulas are polynomial equations, inequations, and inequalities in the $x_i$.  In other words, a problem in $\exists \R$ defines a semialgebraic set over the real numbers and asks whether or not it contains any points \cite{broglia2011lectures}. Many well known problems in computational geometry lie in $\exists \R$, including some problems very similar to determining whether a code is convex. For instance, determining whether a graph is the intersection graph of convex sets in the plane is $\exists \R$ complete \cite{schaefer2009complexity}. 
	
Theorem~\ref{thm:witness} implies the convex code decision problem is at least as difficult as deciding if an oriented matroid is representable.
This decision problem is $\exists\R$-complete \cite{mnev1988universality, shor1991stretchability, sturmfels1987decidability} and therefore the convex code decision problem is $\exists\R$-hard.
	
\begin{introtheorem}
	Any problem in $\exists \R$ can be reduced in polynomial time to the problem of determining whether a neural code is convex. 
\end{introtheorem}
	
\begin{proof}

		
By the Mn\"ev-Sturmfels universality theorem (see \cite{mnev1988universality, sturmfels1987decidability, shor1991stretchability, bjorner1999oriented}), determining whether a uniform oriented matroid is representable is complete for the existential theory of the reals.
By Theorem~\ref{thm:witness}, a uniform oriented matroid $\cM = (E, \cL)$ is representable if and only if $\sfL^\pm(\cM) = \cL \subseteq 2^{\pm E}$ is a convex neural code. Thus problem in $\exists\R$ can be reduced in polynomial time to deciding representability of a uniform oriented matroid and thus convexity of the corresponding code.
\end{proof}

\noindent 
Since any $\exists \R$ complete problem is also $\mathrm{NP}$-hard, we have as a corollary that determining whether a code is convex is $\mathrm{NP}$-hard.
 \begin{cor}
The problem of determining whether a code is convex is $\mathrm{NP}$-hard, where the problem size is measured in the number of codewords. 
\end{cor}
Notice that because we can perform this reduction of a problem in $\exists \R$ to a neural code in polynomial time, this result holds even when we measure the problem size in terms of the number of codewords, which may be exponentially large in the number of neurons.  Again, this NP hardness result is not surprising. For instance, it parallels the result that recognizing whether a simplicial complex is the nerve of convex sets in $\R^d$ is $\mathrm{NP}$-hard for $d\geq 2$ \cite{tancer2010d}.  


	

%\subsection{Matroid completion}
%Results earlier in this paper motivate us to ask the following question: when is a neural code the image of an oriented matroid? More explicitly, given a code $\scC\subseteq 2^{[n]}$, how can we produce an oriented matroid $\cM$ and a code morphism $f$ such that $\scC = f(\cvc(\cM))$, or prove that none exists? Can we do this efficiently? Are there ``matroid code axioms" that the codewords of any code lying below an oriented matroid must satisfy? We state these questions as a ``matroid completion" problem, and note that special cases of this problem have been posed elsewhere in the literature. We define a a matroid completion problem as follows: 
%\begin{prob}
% Given ground set $\pm E$, a set of \emph{forbidden covectors} $F \subseteq 2^{\pm E}$, and $m$ sets of \emph{required covectors}, $R = \{R_1, \ldots, R_k\}$, $R_i \subseteq 2^{\pm E}$, the \emph{matroid completion problem} (E, F, R) asks us to determine whether there exists a matroid $\mathcal M = (E, \mathcal L)$ such that
%\begin{enumerate}
%\item $F\cap \mathcal L = \emptyset $
%\item For each $i\in [k]$, $R_i \cap \mathcal L \neq \emptyset$. 
%\end{enumerate}
%
%\end{prob}
%
%Given a neural code $\scC\subseteq 2^{[n]}$, we can construct a matroid completion problem which has a solution if and only if the $\scC$ is the image of an oriented matroid on $E$ under a morphism which takes at most $m$ elements of $E$ to each element of $[n]$. If this matroid problem has a representable solution,  $\mathcal C$ has a polyhedral realization with $m$ sided convex polytopes. 
%
%Letting $N = mn$ and $E = [N ]$, we construct this matroid completion problem. Define a map $f: [N]\to [n]$ by $f\inv(i) = \{ m(i-1)+1, \ldots, mi\}$. This map $f$ defines a morphism of neural codes $f: 2^{[N]} \to 2^{[n]}$ as the morphism defined by trunks $T_i = \tk_{2^{[N]}}(f\inv(i))$. 
%This morphism can be restricted to any $N$ neuron code $\mathcal D \subset 2^{[N]}$. Given an $n$ neuron code $\mathcal C\subset 2^{[n]}$, we want to choose an oriented matroid $\cM = (E, \cL)$ such that 
%$$\mathcal C = f(\cvc(\cM)).$$
%
%For a fixed morphism $f$ and code $\mathcal C$, we translate this to a matroid completion problem.
%For each $n$ neuron codeword $\sigma \subset 2^{[n]}$, we construct a set of compatible signed sets
%$$S_f(\sigma) = \{ X\in 2^{\pm E} \,  \mid \, X_j= + \mbox{ for all $j$ in $f\inv(i)$ if and only if $i\in \sigma $}\}
%=\cvc\inv (f\inv(\sigma)).$$ 
%Define the set of forbidden covectors $F$ as $$F = \bigcup_{\sigma\notin \scC} S_f(\sigma).$$ Our sets of required covectors are
%$$ R = \{ R_\sigma = S_f(\sigma)\}_{\sigma \in \scC}.$$
%By construction $\scC$ is the image of an oriented matroid on $E$ under the map $f$ if and only if the matroid completion problem $(E, F, R)$ has a solution. Therefore, $\scC$ has a convex realization with $m-$sided polytopes if and only if $(E, F, R)$ has a representable solution. 
%
%\begin{ex} Consider the code $\scC = \{1, 12, 123, 23, 3\}$. First, it is easy to verify using the covector axioms that  $\scC\neq \cvc(\cM)$ for any oriented matroid or affine oriented matroid. In particular, in any realization of $\scC$,  the complement of $U_2$ is disconnected, so $U_2$ cannot be a half space. However, there is no obstruction to $U_1$ and $U_3$ being half spaces. So, to keep the problem as simple as possible,  define the morphism $f: 2^{[4]}\to 2^{[3]}$ by the trunks $T_1 = \tk_{2^{[4]}}(1), T_2 = \tk_{2^{[4]}}(23),$ and $T_3 = \tk_{2^{[4]}}(4)$. 
%
%This defines a the matroid completion problem.
%\begin{align*}
%R_1 &= \{ 1\bar2\bar3\bar 4, 1\bar 2 3 \bar 4, 1 2\bar 3 \bar 4\}\\
%R_{12} &= \{123\bar 4\}\\
%R_{123} &= \{1234\}\\
%R_{23} &= \{\bar 1234\}\\
%R_{3} &= \{ \bar1\bar2\bar3 4, \bar 1\bar 2 3 \bar 4, \bar 1 2\bar 3 4\}\\
%F &= \{\bar1\bar2\bar3\bar4, \bar 12\bar 3\bar 4, \bar 1\bar 2 3 \bar 4, 1\bar2\bar34, 12\bar 34, 1\bar 234, \bar 123\bar 4\}
%\end{align*}
%
%In other words, we require at least one tope to map down to each of the codewords $1, 12, 123, 23, 3$ and forbid codewords which map to $\emptyset, 13$, or $2$. The required codeword $ 1234$ forces the matroid to be acyclic, so we can assume the positive part of each covector is also the positive part of a tope. 
%
%This matroid completion problem is small enough to solve by brute force.  We know we must take $R_{12} \cup R_{123} \cup R_{23} \subset \cW$, since these required sets each contain only one element. Now, we pick some elements from $R_1$ and $R_3$ arbitrarily. For instance,  choose $\{1\bar 23\bar 4\}$ from $R_1$ and $\{\bar 1 2 \bar 3 4\}$ from $R_3$. (There are few enough elements that we can test all subsets of $R_1$ and $R_3$ in a reasonable amount of time.)
%
%Using Da Silva's axioms for topes of oriented matroids \cite{dasilva1987, dasilva1991}, we check whether  $\cW = \{123\bar4, 1234, \bar 1234, 1\bar234, \bar 12\bar 34\}$ is the set of topes of an affine oriented matroid. It is. 
%\end{ex}
%
%This brute force method quickly becomes impractical as the sizes of $\scC$ and $E$ increase. Thus, we ask the following: 
%
%\begin{question}
%Is there an efficient algorithm to solve the matroid completion problem $(E, F, R)$ arising from a neural code $\scC$ and morphism $f$?  Is there an efficient algorithm to solve general matroid completion problems?
%\end{question}
%Since we know from the previous section that checking convexity is $\mathrm{NP}$-hard, we may be somewhat loose in our definition of efficient.  Similarly, we ask whether there is a good way to characterize when a matroid completion problem has a solution. 
%\begin{question}
%Are there simple combinatorial criteria which determine when the matroid completion problem $(E, F, R)$ has a solution?
%\end{question}
%
%Similar problems have been posed elsewhere in the literature. For instance, \cite{bandelt2018coms} define a conditional oriented matroid (COM) as a set of signed subsets satisfying a modified version of the cocircuit axioms. COMs are intended to axiomatize the sets of signed sets which arise from intersecting a convex set with a hyperplane arrangement. Thus, every realizable COM arises as a fiber of a representable oriented matroid. (In our language, this says that every COM is a trunk in some representable oriented matroid.) As Conjecture 1, the authors of \cite{bandelt2018coms} ask whether any COM is a trunk in an oriented matroid. We can phrase this as a matroid completion problem. Let $\scC$ be the covectors of a COM on ground set $E$. We ask whether $\scC$ is a trunk of an oriented matroid  $\cM = (E\cup G, \cL)$. For each $X\in \scC$, let $R_X = \{ X\cup G\}$. In other words, each covector of $\scC$ must appear as a covector of $\cM$ containing $G$ in its positive part.  The set of forbidden covectors is the set $F = \{ Y\cup G  \mid  Y\notin \scC\}$. In other words, the only covectors with $F$ in their positive part must be the covectors of $\scC$, since we want to obtain $\scC$ from $\cL$ by taking the trunk of $F$. Thus, Conjecture 1 of  \cite{bandelt2018coms} can be rephrased as follows: 
%\begin{conjecture} [Conjecture 1 of \cite{bandelt2018coms}]
%If $\scC$ satisfies the COM covector axioms, then there is some finite set $G$ such that the matroid completion problem $(E\cup G, F,  \{R_X \mid  X\in \scC\})$ has a solution. 
%\end{conjecture}




